Evolution of a Pulsar Wind Nebula within a Composite Supernova Remnant

The interaction between a pulsar wind nebula (PWN) and its host supernova remnant (SNR) can produce a vast array of observable structures. Asymmetry present within these structures derives from the complexity of the composite system, where many factors take turns playing a dominating hand throughout the stages of composite SNR evolution. Of particular interest are systems characterized by blastwave expansion within a nonuniform interstellar medium (ISM), which contain an active pulsar having a substantial "kick" velocity (upward of 300 km s$^{-1}$ ), because these systems tend to produce complex morphologies. We present a numerical model that employs these and several other factors in an effort to generate asymmetry similar to that seen in various X-ray and radio observations. We find that the main parameters driving structure are ISM uniformity and total pulsar spin- down energy, with secondary contributions from factors such as pulsar trajectory and initial spin-down luminosity. We also investigate the dynamics behind PWN "tails," which may form to link active pulsars to a crushed, relic nebula as the reverse shock passes. We find that the directions of such tails are not good indicators of pulsar motion, but direction does reveal the flow of ejecta created by the passage of a reverse shock.

==> parameters.tex <==
%------------------------------------------------------------------------------
% Include :: Model Parameters
%------------------------------------------------------------------------------

\begin{table*}[t]
  \begin{center}
  \begin{tabular}{c}	% main table
  \textbf{Model Parameters}  \\ [0.25em]
  \hline
  \hline \\
  \begin{tabular}{c | c c c c c c c c}

   % Headers
   			&
   Explosion		&
   Ejecta mass 		&
   Spin-down 		&
   Spin-down 		&
   Pulsar kick 		&
   Pulsar kick 		&
   Asymptotic 		&
   Characteristic	  \\ 

   % Headers (line 2)
   			&
   energy 		&
			&  
   luminosity		&
   timescale		& 
   velocity		& 
   direction 		&
   density ratio	& 
   length scale		  \\ [0.2em]


   			&
   ($10^{51}$ erg) 	&
   ($M_\odot$) 		&
   ($10^{38} \text{erg s}^{-1}$) &
   (kyr) 		&
   (km s$^{-1}$) 	&
   (\textit{radians})	&
    			&
   ($10^{18}$ cm) 	  \\ [0.1em]


   Model		&
   $E_{51}$		&
   $M_\text{ej}$	&
   $L_\text{p}(0)$	& 
   $\tau$		& 
   $v_\text{psr}$	& 
   $\psi_\text{kick}$	&
   $(x-1)^{-1}$		& 
   $H$			  \\ 
   \hline


  % Model A :: 'The Eye'
  % run available in 'pwnsnr_research/nov19_velplot_tests/run01_eye/'
  % -------------------------
    A 			&
    0.5 		&
    4.5 		&
    2.8 		&
    2.0 		&
    350 		&
    $3\pi/4$ 		&
    12.5 		&
    1.6 		  \\ [0.1em]
%   0.314


  % Model B :: Not Updated
  % run available in ??
  % -------------------------
    B 			&
    1.0 		&
    4.0 		&
    2.8 		&
    2.0 		&
    350 		&
    $\pi/4$ 		&
    20.0 		&
    30 			  \\ [0.1em]
%   0.018


  % Model C :: Not Updated
  % run available in ??
  % -------------------------
    C 			&
    1.0 		&
    3.5 		&
    1.0 		&
    0.75		&
    300 		&
    $3\pi/8$ 		&
    10.0 		&
    3.0 		  \\ [0.1em]
%   0.160


  % Model D :: Tail Directions
  % run available in 'pwnsnr_research/jun04_tail_comparison/*',
  %                  'pwnsnr_research/nov28_tail_comparison/*'
  % -------------------------
    D 			&
    1.0 		&
    4.5 		&
    2.8 		&
    1.5 		&
    500 		&
    *\textit{variable} 	&
    12.5 		&
    12  		  \\ [0.1em]
%   0.042


  % Model E :: Not Updated
  % Run Available in ??
  % -------------------------
    E 			&
    1.0 		&
    4.5 		&
    2.8 		&
    1.5 		&
    500 		&
    $7\pi/8$ 		&
    12.5 		&
    12			  \\ [0.1em]
%   0.042

  \end{tabular}
  \end{tabular}
  \end{center} 
\caption{	\label{parameters}}%Needs to be updated/organized}
\end{table*}

